Char2Subword: Extending the Subword Embedding Space Using Robust Character Compositionality

Byte-pair encoding (BPE) is a ubiquitous algorithm in the subword tokenization process of language models as it provides multiple benefits. However, this process is solely based on pre-training data statistics, making it hard for the tokenizer to handle infrequent spellings. On the other hand, though robust to misspellings, pure character-level models often lead to unreasonably long sequences and make it harder for the model to learn meaningful words. To alleviate these challenges, we propose a character-based subword module (char2subword) that learns the subword embedding table in pre-trained models like BERT. Our char2subword module builds representations from characters out of the subword vocabulary, and it can be used as a drop-in replacement of the subword embedding table. The module is robust to character-level alterations such as misspellings, word inflection, casing, and punctuation. We integrate it further with BERT through pre-training while keeping BERT transformer parameters fixed--and thus, providing a practical method. Finally, we show that incorporating our module to mBERT significantly improves the performance on the social media linguistic code-switching evaluation (LinCE) benchmark.

==> sections/2-methodology_old.tex <==
\section{Method}
% \tn{Maybe phrase this as "token" vs. "subtoken"? E.g. the double-question mark is a token, but not a word, which can be broken into two subtokens (i.e. two single question marks).}
Given a word $w$, a subword model produces a sequence of subword pieces $\vs = (s_0, s_1, \dots, s_n)$, such that the concatenation of all the segments from $\vs$ fully reconstructs the word $w$. 
% Note that the length of a subword piece $s_i$ can go from one character to all the characters of the word $w$.
% However, 
Regardless of whether a subword piece represents a character in a word or not, all the pieces are treated as semantic units within a sentence.\footnote{Previous studies \citep{clark-etal-2019-bert,rogers2020primer} have shown that BERT abstracts linguistic properties such as syntax and parsing within its self-attention probabilities. That is evidence that subwords need to preserve some semantics when fed into such layers. This suggests that subword pieces broken down to the character level can prevent the model from exploiting linguistic properties.} 
Such pieces come from a rule-based system that does not take into account semantics or morphology during the tokenization.
Thus, the subword tokenization has a significant impact on the semantic abstraction from upper layers in pre-trained models like mBERT.
% This happens in current transformer-based models, where their strict tokenization into subword pieces has a significant impact on the semantic abstraction of upper layers of the model. 
% A rule-based system generates the tokenization without taking any semantics into account \citep{he-etal-2020-dynamic}. 
% This makes it hard to guarantee that the resulting tokenization is optimal for the model to interpret the underlying semantics of the sentence. 
% \tn{Let's add discussions on how those tokenization is obtained -- it is through a rule-based system without taking any semantics into account. This makes it hard to guarantee that the resulting tokenization is optimal for the model to interpret the underlying semantics of the sentence. 
% % Btw, it might be helpful to discuss this previous work: https://arxiv.org/pdf/2005.06606.pdf -- its good and bad.
% }

% Such semantic sequence is usually preserved throughout all the layers of a transformer-based model without hierarchically distinguishing their linguistic roles (e.g., a serie of character pieces within a word hardly contributes at the semantic level)
To alleviate such problems, we build word representations out of characters.
The character-to-subword (char2subword) module allows flexible tokenization patterns, where the model can split by spaces, use the original tokenization method, or employ a different tokenization process as defined by the user.
There are two main phases in our proposed method: approximating 
subword embeddings with the char2subword module (i.e., ideally replicating the embedding space $\mE$) (Section \ref{ch9:sec:ch2sw_mimic}), and contextually integrating the char2subword module into the pre-trained model (Section \ref{ch9:sec:ch2sw_pretrain}).
% \tn{here maybe use a little more words to define "simulate"} 


% ====================================================
% MIMICKING
% ====================================================
\subsection{Approximating the subword embedding} 
\label{ch9:sec:ch2sw_mimic}

% Embedding representations from BERT-like models rely on subword vectors.
% We aim at replacing the embedding lookup table by introducing a more meaningful mechanism,\footnote{Instead of simply retrieving subword vectors, this mechanism makes better use of the parameters in the embedding table by handling rare character sequences while still preserving the meaning of the words.} the character-to-subword module. 
% This module is trained from scratch to mimic the vectors from the embedding lookup table using the characters of the vocabulary words. 

Consider a subword $s_i$ from the vocabulary $\mathcal{V}$ and a subword embedding matrix $\mE \in \sR^{|\mathcal{V}|\times d}$. 
We learn a parameterized function $f_\theta: \sR^{|c| \times 1} \rightarrow \sR^d$ that maps the sequence of characters $\vc_i = (c_{i1}, c_{i2}, \dots, c_{i|s_i|})$ from the subword $s_i$ to its corresponding embedding vector $\ve_i \in \mE$:
\begin{align*}
    \hat{\ve_i} = f_\theta(\vc_i) ~~~s.t.~~ \hat{\ve}_i \approx \ve_i
\end{align*}
To accomplish that, we optimize $f_\theta$ by minimizing the overall objective function $\mathcal{L}(\cdot)$:
\begin{gather+}[0.93]
\mathcal{L}(\vc_i, \ve_i, \vy_i, f_{\theta}) =
    \mathcal{L}_{cos}(\ve_i, f_{\theta}(c_i)) + \normltwo(\ve_i, f_{\theta}(c_i)) \\
    ~~~~~~~~~~~~~~~~~~~~~~~~~~~
    + \mathcal{L}_{nbr}(\ve_i, f_{\theta}(c_i)) + 
    \mathcal{L}_{ce}(\vy_i, f_{\theta}(c_i))
    % \mathcal{L}_{ce}(\vy_i, \hat{\vy}_i)
\end{gather+}
% \begin{equation}
% \resizebox{\hsize}{!}{%
% $$
% \mathcal{L}(\vc_i, s_i, \ve_i, f_{\theta}) 
% = \mathcal{L}_{cos}(\ve_i, f_{\theta}(c_i)) + \normltwo(\ve_i, f_{\theta}(c_i)) + \mathcal{L}_{nbr}(\ve_i, f_{\theta}(c_i)) + \mathcal{L}_{ce}(s_i, f_{\theta}(c_i)) \notag
% $$
% }
% \end{equation}
% \begin{align}
% \mathcal{L}(\vc_i, s_i, \ve_i, f_{\theta}) 
%     =~& \mathcal{L}_{cos}(\ve_i, f_{\theta}(c_i))  \notag \\
%       &+~\mathcal{L}_{ce}(s_i, f_{\theta}(c_i))    \notag \\
%       &+~\normltwo(\ve_i, f_{\theta}(c_i))         \notag \\
%       &+~\mathcal{L}_{nbr}(\ve_i, f_{\theta}(c_i)) \notag
% \end{align}

% where $\lambda_1$, $\lambda_2$, and $\lambda$ are scalars to weight down or up the losses. 

The first objective, $\mathcal{L}_{cos}(\cdot)$, is the cosine distance between the target and the predicted embedding vectors $\ve_i$ and $\hat{\ve}_i$. 
By using an angular distance function, we encourage the model to replicate the semantic relationships and vector arrangements in the original embedding space of $\mE$:
% \footnote{This objective is very important since our goal is to replicate embedding vectors that are similar to $\mE$ so that our model is compatible with upper layers of the full pre-trained transformer-based model.}
\begin{align*}
    % \mathcal{L}_{cos}(\ve_i, \hat{\ve}_i) =~1 - cos(\ve_i, \hat{\ve}_i)
    \mathcal{L}_{cos}(\ve_i, \hat{\ve}_i) = ~1 - \frac{\ve_i \cdot \hat{\ve}_i}{||\ve_i|| ~||\hat{\ve}_i||}
\end{align*}
% \tn{Looks like some eqs are numbered while the others are not.}

The second objective is the cross-entropy loss $\mathcal{L}_{ce}(\cdot)$.
We use $\mE$ as fixed parameters to project linearly from the embedding to the vocabulary space.
This loss term forces the model to learn accurate embedding representations such that they map to the original subwords from the vocabulary $\mathcal{V}$:
\begin{align*}
% \mathcal{L}_{ce}(s_i, \hat{\ve}_i) = -s_i \log p(\hat{\ve}_i \cdot \mE^\top) %~~~s.t.~~ s_i \in {0,1}^n 
% \mathcal{L}_{ce}(\vy_i, \hat{\vy}_i) &= -\sum^{|\mathcal{V}|}_j \vy_{ij} \log \hat{\vy}_{ij} \\
\mathcal{L}_{ce}(\vy_i, \hat{\ve}_i) &= -\sum^{|\mathcal{V}|}_j \vy_{ij} \log \hat{\vy}_{ij} \\
% \mathcal{L}_{ce}(\vy_i, \hat{\ve}_i) &= -\log \hat{\vy}_{ij} \\
s.t. ~~~\hat{\vy}_i &= \softmax(\hat{\ve}_i \cdot \mE^\top)
% \mathcal{L}_{ce}(s_i, \hat{\ve}_i) = -\sum^{|\mathcal{V}|}_j \vy_{ij} \log \mathrm{softmax}(\hat{\ve}_i \cdot \mE^\top)_j
\end{align*}

The third objective is the $\normltwo$ norm or euclidean distance between the vectors $\ve_i$ and $\hat{\ve}_i$.
The previous objectives do not regulate the magnitude of the predicted vector $\hat{\ve}_i$, allowing that to be a degree of freedom for $f_\theta$.
By using the $\normltwo$ norm, we penalize the model for generating a vector $\hat{\ve}_i$ with a different magnitude than $\ve_i$. 
% \tn{If we don't have a dedicated ablation study on this, we might need to state a bit more the motivation of this term -- why keeping the same magnitude is important.}
Regulating the magnitude is important to approximate the vector arrangements in the embedding space. 
We hypothesize that slightly different properties in the embedding $\mE$ can magnify differences at the upper layers of mBERT.

The last objective, $\mathcal{L}_{nbr}(\cdot)$, is the mean squared error (MSE) of cosine distances
% \footnote{Defined as $dis(\va, \vb) = 1 - cos(\va, \vb)$ where $\va, \vb \in \sR^d$.} 
generated between the $k$-th closest neighbors to $\ve_i$ versus the distances of the same neighbors with respect to $\hat{\ve}_i$:
% \begin{align*}
%     (\vn_1, \dots \vn_k) =&~ topk(\ve_i, \mE) \\
%     \mathcal{L}_{nbr}(\ve_i, \hat{\ve}_i) =&~ \frac{1}{k}\sum_{j=1}^k{( dis(\ve_i, \vn_j) - dis(\hat{\ve}_i, \vn_j)  )^2}
% \end{align*}
\begin{gather+}[0.93]
    (\vn_1, \dots \vn_k) =~ topk(\ve_i, \mE) ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\\
    \mathcal{L}_{nbr}(\ve_i, \hat{\ve}_i) =~ \frac{1}{k}\sum_{j=1}^k{( dis(\ve_i, \vn_j) - dis(\hat{\ve}_i, \vn_j)  )^2}
\end{gather+}
where $topk(\cdot)$ retrieves the $k$-th closest neighbors according to the cosine distances among all the subword vectors in $\mE$.
The main idea of this objective is to force distances between $\hat{\ve}_i$ and the neighbors $\vn_*$ to be as similar as possible to the distances between the same neighbors and $\ve_i$.

\begin{figure}[t!]
\centering
\includegraphics[width=\linewidth]{images/naacl_char2subword2.jpg}
\caption{
The char2subword module approximates the mBERT subword embedding table.
We incorporate noise in every word with single-character operations. 
    % The char2subword module is trained using the subword embedding lookup table from a pre-trained language model (e.g., mBERT). We incorporate noise in every word at the character level with single-character operations. 
    % \tn{Let's make the figure a little bigger.}
}
\label{ch9:fig:char2subword}
\end{figure}
\begin{table}[t!]
\small
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lp{2.2in}}
    \toprule
    \bf Operation & \bf Description \\
    \midrule
    \texttt{mistype} & replace a random character of a subword by randomly choosing from its nearby keys according to a keyboard layout \\
    \midrule
    \texttt{repeat} & repeat a random character of a subword \\
    \midrule
    \texttt{swap} & randomly choose a character and swap it with the next character in a subword \\
    \midrule
    \texttt{drop} & randomly drop a character of a subword \\
    \midrule
    \texttt{toggle} & toggle the case of a randomly chosen character from a given subword \\
    \midrule
    \texttt{punct} & randomly add a punctuation mark commonly used within words (e.g., dashes, periods) \\
    \bottomrule
\end{tabular}
}
\caption{
% \tn{Let's also drop all periods (the punctuations) in the table:)} 
Single-character operations to incorporate noise in the approximation stage. 
The operations are applied to every word in the vocabulary that exceeds the four characters. % and that it is not a special token.
% \tn{I would use first person verb "replace" instead of "replaces"; so are the rest.}
}
\label{ch9:tab:noise_operations}
\end{table}

% \tn{I would suggest using paragraph instead of subsubsection}
\paragraph{Char2subword module} 
% \subsubsection{The Char2subword Module}
% \label{ch9:sec:ch2sw_architecture}
% \tn{Maybe write this out like "$c_i=(c_{i1}, c_{i2}, ..., c_{iM})$"?} 
We model $f_\theta$ using the transformer architecture \citep{vaswani2017attention}.
The module processes a sample as a sequence of characters $\vc_i = (c_{i1}, c_{i2}, \dots, c_{iM})$ 
of a subword $s_i$ of length $M$.\footnote{
To distinguish between words and subwords, we prepend `\#\#' to the sequence $\vc_i$ in the case of full words.
}
We represent the sequence $\vc_i$ as the sum between the character embeddings and sinusoidal positional encodings.
We pass the resulting sequence of character vectors $\mX_0$ to a stack of $l$ attention layers, each with $k$ attention heads. On top of the $l$ attention layers, we add a linear layer $\mW_e \in \sR^{d' \times d}$ followed by max-pooling and a layer normalization for the final output $\hat{\ve}_i$ (see full definition in Appendix \ref{app:char2subword_definition}).

\paragraph{Character-level robustness}
% \subsubsection{Character-level robustness}
% \label{sec:}
% The flexibility of the char2subword module $f_\theta$ allows introducing robustness at the character level 
% \tn{
The flexibility of the char2subword module makes it easier to teach the model text invariance because the inputs are now processed at the character-level.
% }. 
We augment the subword vocabulary $\mathcal{V}$ by introducing natural single-character misspellings during training. 
We apply one operation at a time and only to subwords that exceed four characters to reduce the chance of ambiguity between valid subwords.
The operations are described in Table \ref{ch9:tab:noise_operations} and the high-level view of the approximation appears in Figure \ref{ch9:fig:char2subword}.\footnote{
For the \texttt{mistype} operation, we use over 100 keyboard layouts to cope with the languages in mBERT.
}


% ====================================================
% PRE-TRAINING
% ====================================================
\subsection{Pre-training with the char2subword}
\label{ch9:sec:ch2sw_pretrain}

The previous techniques leverage the pre-trained knowledge in the embedding matrix $\mE$. 
However, the char2subword module may not be integrated with the pre-trained mBERT's upper layers since it has only seen individual subwords without context.
To alleviate that, we pre-train the char2subword module along with mBERT \citep{gururangan-etal-2020-dont}. 
We do not update parameters in upper layers of mBERT since the goal is to provide the char2subword module as a drop-in alternative for $\mE$ on the publicly available pre-trained models.\footnote{
While the study focuses on mBERT, this method can be applied to other pre-trained models like RoBERTa or XLM-R.
}

Following \citet{liu-etal-2019-roberta}, we use a dynamic masked language modeling (MLM) objective (see Figure \ref{ch9:fig:pretraining}).
We randomly choose 15\% of the subword tokens and mask them at the character level. 
We replace 80\% of the characters with \texttt{[MASK]}, 10\% with randomly chosen characters and the remaining 10\% is left unchanged.
We feed characters to the char2subword module and make predictions from the subword vocabulary $\mathcal{V}$.\footnote{
% Using the pre-trained embedding table $\mE$, 
We project the internal representations per word onto the vocabulary space using $\mE$ (without updating its parameters).
}
We pre-train the char2subword model with 1M sequences of 512 subword tokens from Wikipedia (200K sequences for each English, Spanish, Hindi, Nepali, and Arabic text).
Using gradient accumulation, we update parameters with an effective batch size of 2,000 samples.
Note that the model does not require extensive pre-training since 1) the upper-layer parameters are initialized from the pre-trained mBERT checkpoint and kept fixed during training, and 2) the char2subword module is initialized from the embedding approximation phase.
Thus, pre-training the model for a few epochs is sufficient.
% \footnote{
% we pre-train this model for 3 epochs using distributed training over 32 Tesla V100 GPUs. The model takes about a day to complete one epoch.
% }

\begin{figure}[t!]
\centering
\includegraphics[width=\linewidth]{images/naacl_pretraining2.jpg}
% \includegraphics[width=\linewidth]{images/naacl_pretraining.png} % Use this one for more space
\caption{
An example of an input and output of the pre-training setting with a masked language modeling (MLM) objective at the character level.
}
\label{ch9:fig:pretraining}
\end{figure}

% Note that the flexibility of applying this method enables the model to enhance its original vocabulary. 
% That is, with words built from characters 
% Importantly, this method allows to enhance the embedding space already captured by mBERT with the opportunity to 

% ====================================================
% FINETUNING
% ====================================================
\subsection{Fine-tuning}
\label{ch9:sec:ch2sw_finetune}

Once the char2subword module has been optimized, we evaluate the pre-trained model with the char2subword module on downstream NLP tasks.
Specifically, we experiment with two scenarios: the full and the hybrid modes. 

% \tn{Maybe rephrase? Imo we're not replacing the "table", but rather the whole set of embedding vectors/parameters.} 
\paragraph{Full mode} 
This mode completely replaces the subword embedding table in mBERT (i.e., the set of parameters and vectors) with the char2subword module.
% (see Figure \ref{ch9:fig:finetuning_scenarios} (center)).
The idea of this setting is to evaluate how well approximated was the embedding space originally in $\mE$.
Intuitively, if the char2subword replicates the embedding space in $\mE$ perfectly, then the overall model should behave about the same as the original mBERT model.
Nevertheless, this setting does not tokenize further a word; hence, the input sequence tends to be shorter and more meaning-preserving (i.e., too many subword pieces for a single word can degrade its meaning).
% This setting should be able to both overcome mispellings while also preserving the original knowledge in the embedding table without splitting dramatically subwords into multiple pieces.

% \begin{figure*}[!ht]
% \centering
% \includegraphics[width=3.5in]{images/finetuning_scenarios.png}
% \caption{
%     The fine-tuning scenarios with the char2subword module. 
%     % \textbf{Full mode} refers to subword embedding table replaced with a char2subword module. 
%     % \textbf{Hybrid mode} refers to the character back-off strategy where both subword and character-based embeddings are used. 
%     % \textbf{Detached mode} refers to a text-level preprocessing before passing the inputs to the original model.
%     The mBERT model structure (left) is added for reference.
%     The full mode (center) shows the char2subword module instead of the subword embedding table.
%     The hybrid mode (right) represents both the subword embedding table and the char2subword module. 
%     The char2subword module is only used when the input word does not appear in the vocabulary as a whole.
%     % \tn{The two emtpy boxes in the right figure (bottom) looks a little confusing to me.}
% }
% \label{ch9:fig:finetuning_scenarios}
% \end{figure*}

\paragraph{Hybrid mode} 
Unlike the full mode, this mode does not replace the subword embedding table. % (see Figure \ref{ch9:fig:finetuning_scenarios} (right)). 
Instead, it uses the subword embedding vectors by default for full words (i.e., not subword pieces). The model backs off to character-based embeddings from the char2subword module when a word as a whole does not appear in the vocabulary.
This method focuses specifically on subwords rather than full words, effectively preventing words from being broken down into pieces.
% This method prevents words to be broken down into pieces by building word representations out of its characters.

% \begin{figure}[h!]
% \centering
% \includegraphics[width=4in]{images/char-backoff.png}
% \caption{
% An example of the character backoff strategy. The only word that is passed to the char2subword module is \textit{nanotechnology}; the rest is embedded using the subword embedding table.
% }
% \label{ch9:fig:char_backoff}
% \end{figure}




==> tables/finetuning_test_results.tex <==

\begin{table*}[h!]
    \small
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l|c|cccc|cc|ccc}
    \toprule
     & 
     & \multicolumn{4}{c|}{\textbf{LID }}    % (Weighted F1)
     & \multicolumn{2}{c|}{\textbf{POS}}    % (Accuracy)
     & \multicolumn{3}{c}{\textbf{NER}} \\   % (Micro F1)
    \textbf{Method} 
        & \textbf{Avg}
        % & \textbf{SPA-ENG} & \textbf{HIN-ENG} & \textbf{NEP-ENG} & \textbf{MSA-EA}  % LID
        % & \textbf{SPA-ENG} & \textbf{HIN-ENG} 
        % & \textbf{SPA-ENG} & \textbf{HIN-ENG} & \textbf{MSA-EA}  \\  % NER
        % & SPA-ENG & HIN-ENG & NEP-ENG & MSA-EA  % LID
        % & SPA-ENG & HIN-ENG 
        % & SPA-ENG & HIN-ENG & MSA-EA  \\  % NER
        & es-en & hi-en & ne-en & msa-ea  % LID
        & es-en & hi-en 
        & es-en & hi-en & msa-ea  \\  % NER
    \midrule
    mBERT 
    & 85.09 & 98.36  & 94.24  & 96.32  & 91.55 & 97.07	 & 86.30 & 64.05  & 72.57  & 65.39  \\
    % \midrule
    Best proposed model  
    & \textbf{85.69} & 98.33  & 96.23  & 96.19  & 91.19 & 96.88  & 88.23  & 64.65  & 73.38  & 66.13  \\
    \bottomrule
    \end{tabular}}
    \caption{
    Results on the test set of the LinCE benchmark using the hybrid char2subword mBERT model (best proposed model). 
    The languages involved are English (en), Spanish (es), Hindi (hi), Nepali (ne), Modern Standard Arabic (msa), and Egyptian Arabic (arz).
    The scores for LID, NER, and POS are weighted F\textsubscript{1}, micro F\textsubscript{1} with spans, and accuracy, respectively.
    State of the art as of October 19th, 2020: \texttt{https://ritual.uh.edu/lince/leaderboard}.
    }
    \label{ch9:tab:lince_test_results}
\end{table*}
